Diffusing Graph Attention

The dominant paradigm for machine learning on graphs uses Message Passing Graph Neural Networks (MP-GNNs), in which node representations are updated by aggregating information in their local neighborhood. Recently, there have been increasingly more attempts to adapt the Transformer architecture to graphs in an effort to solve some known limitations of MP-GNN. A challenging aspect of designing Graph Transformers is integrating the arbitrary graph structure into the architecture. We propose Graph Diffuser (GD) to address this challenge. GD learns to extract structural and positional relationships between distant nodes in the graph, which it then uses to direct the Transformer's attention and node representation. We demonstrate that existing GNNs and Graph Transformers struggle to capture long-range interactions and how Graph Diffuser does so while admitting intuitive visualizations. Experiments on eight benchmarks show Graph Diffuser to be a highly competitive model, outperforming the state-of-the-art in a diverse set of domains.

==> discard.tex <==
\begin{figure}
    \begin{tabular}{cc}
        \includegraphics[scale=0.42]{images/attention_combine.pdf}\label{combine_attention} &
        \includegraphics[scale=0.42,trim={4 0 0 0}, clip]{images/fig_example.pdf}\label{graph_input} \\
        \small{(a)} & \small{(b)}
    \end{tabular}

    \caption{(a)~Example of a 5x5 grid. The label for node 23 is 1, since it matches only with node 20, and the label for node
    12 is 3, since it matches with nodes 11,13,17.
        (b)~visualization of the position and content attention our trained model gives to node \textcolor{red}{23}
        in the input shown in (a). The models learns to pay attention to nodes in the same row and column using the positional attention and to nodes of the same color using the content attention. Their element-wise product selects only the nodes that are relevant for solving the task.
    }
\end{figure}



==> reproduce.tex <==
\paragraph{REPRODUCIBILITY STATEMENT}
The authors support and advocate the principles of open science and reproducible research.
We describe Graph Diffuser in detail in the text and figures and mention all relevant hyperparameters to reproduce our experiments in the appendix. Moreover, we will release our code as open-source with clear instructions on how to reproduce all of our results, as well as how to extend our model and apply it to new datasets.

